Teaching Drones on the Fly: Can Emotional Feedback Serve as Learning Signal for Training Artificial Agents?

We investigate whether naturalistic emotional human feedback can be directly exploited as a reward signal for training artificial agents via interactive human-in-the-loop reinforcement learning. To answer this question, we devise an experimental setting inspired by animal training, in which human test subjects interactively teach an emulated drone agent their desired command-action-mapping by providing emotional feedback on the drone's action selections. We present a first empirical proof-of-concept study and analysis confirming that human facial emotion expression can be directly exploited as reward signal in such interactive learning settings. Thereby, we contribute empirical findings towards more naturalistic and intuitive forms of reinforcement learning especially designed for non-expert users.

==> simulations.tex <==
\section{Simulations}
\label{sec:simulations}

We first present some experiments on simulated data, which allows us to systematically study the overall difficulty of the learning problem, as well as the impact of the different types of error sources, such as errors in the feedback classifications or users' difficulty in expressing the right type of feedback (i.e., \emph{feedback error}), or misclassifications in the command recognition module (i.e., \emph{command recognition error}).

We simulate real users' capacity in conveying their "satisfaction" with the drone's chosen actions in a probabilistic way. Thus, various users can be simulated with a \emph{varying capability of providing feedback}.

To simulate our users' behavior, we thus will generate a \texttt{User Agent}, $\mathcal{U}$, which mocks real users' behavior.

Users:
\begin{itemize}
    \item define their desired command-action mapping $f(\Co) = \Ac$
    \item show a command $\co \in \Co$ to the drone
    \item provide feedback on how satisfied they were with the drone's chosen action $\ac \in \Ac$
    \item have different rates of success in conveying their response emotionally, as well as emotional expressivity
\end{itemize}

We assume that each user $u_i$ has a different "success rate" for communicating their (dis)satisfaction to the drone - i.e., here, we probabilistically model the user's expressivity as well as noise in \textsc{fer}'s classification accuracy.

We define for each user some probability distribution, on how capable s/he is in expressing whether s/he's (dis)satisfied with the drone's chosen action: 
\begin{align}
    \mathcal{P}_{success} (u_i) & =  \mathcal{P}\,( u_i = pos.emotion | u_i = satisfied) \\ & =  \mathcal{P}\,( u_i = neg. emotion | u_i = \lnot satisfied)    
\end{align}

A success rate of 60\%, for example, means that in 60\% of the cases we sample from the positive emotions if the chosen action corresponded to the user's intended action, and 40\% we sample from the negative ones.

We also define an "expressivity" degree $\mathcal{P}_{expressivity}(u_i)$, which should model how "expressive" a user $u_i$ is in its mimic. This should regulate how well the user's emotional expression can be distinguished, i.e., how "well-separated'' positive and negative emotions are.

\begin{figure}[h]
	\centering
	\includegraphics[width=0.6\columnwidth]{figures/user_sim_pos.pdf}
	\includegraphics[width=0.6\columnwidth]{figures/user_sim_neg.pdf}
	\label{fig:usim}
	\caption{Examples of simulated positive and negative user feedback, respectively.}
\end{figure}
Fig.~\ref{fig:usim} shows an example of such generated user feedback. We note that these (\emph{stationary}!) distributions are an overly simplistic assumption and look quite different than the distributions we obtain from analyzing real video streams with \textsc{fer} (in which the emotion classes appear much more separated, which will be beneficial for our purposes). For our first simple analysis, we will continue with this simplified setting.

We start under the assumption that \textbf{gesture recognition} works \textbf{perfectly} - i.e., we always correctly recognize the shown command (and thus always will update the correct bandit associated with the recognized gesture). However, there still may be errors in the facial emotion recognition, which will complicate the learning problem.

\begin{figure}[h]
	\centering
	\includegraphics[width=\columnwidth]{figures/sim01.png}
	\includegraphics[width=\columnwidth]{figures/sim01_2.png}
	\includegraphics[width=\columnwidth]{figures/sim01_3.png}
	\label{fig:sim01}
	\caption{Simulation result for a \texttt{UserAgent} generated with parameters $\mathcal{P}_{success} = 0.8$, $\mathcal{P}_{expressivity} = 0.9.$, gesture recognition error rate = $0$. Rows: Results for each of the different gestures, i.e., bandits. Left column: Action values ($Q$) -- ideal result: The value for the correct action (\textbf{ground truth} from the \texttt{UserAgent}'s internal mapping; indicated by a thickened line) should be high, for incorrect actions (dotted lines) low. Right column: Action selection counts $n$. Time steps with \textbf{\emph{feedback errors}} are highlighted with \textbf{red background}.}
\end{figure}
Fig.~\ref{fig:sim02} shows the result of one experiment with one \texttt{UserAgent} with 30 trials, depicting the evolution of  \emph{Q-values} and action selection counts over time. 
%As we can observe, for each gesture, learning converges towards the correct action having the \emph{highest Q-value} after a few trials. 
For better interpretability, time steps where \emph{erroneous feedback} was given or computed are shaded with a red background color on the Q-value plot, which highlights when Q-values were modified possibly "in the wrong direction" (according to the ground truth, i.e., the desired mapping), thus decrease the correct action's value or increase incorrect action's value. 

\begin{figure}[t]
	\centering
	\includegraphics[width=\columnwidth]{figures/sim02_expr04.png}
	\includegraphics[width=\columnwidth]{figures/sim02_expr04_2.png}
	\includegraphics[width=\columnwidth]{figures/sim02_expr04_3.png}
	\label{fig:sim02}
	\caption{Simulation result for a \texttt{UserAgent} generated with parameters $\mathcal{P}_{success} = 0.8$, $\mathcal{P}_{expressivity} = 0.4.$, gesture recognition error rate = $0$. Visualization settings are the same as in Fig.~\ref{fig:sim01}. With lower expressivity, the $Q$-values of the different actions appear less separated.}
\end{figure}

\begin{figure}[t]
	\centering
	\includegraphics[width=\columnwidth]{figures/sim_03_succ06.png}
	\includegraphics[width=\columnwidth]{figures/sim_03_succ06_2.png}
	\includegraphics[width=\columnwidth]{figures/sim_03_succ06_3.png}
	\label{fig:sim03}
	\caption{Simulation result for a \texttt{UserAgent} generated with parameters $\mathcal{P}_{success} = 0.6$, $\mathcal{P}_{expressivity} = 0.9.$, gesture recognition error rate = $0$. Visualization settings are the same as in Fig.~\ref{fig:sim01}. With more \emph{feedback errors}, estimating the correct $Q$ values naturally becomes increasingly difficult.}
\end{figure}

Figs.~\ref{fig:sim02} and \ref{fig:sim03} show results with different \texttt{UserAgent} parameters, but still assuming perfect gesture recognition. Conversely, Fig.~\ref{} assumes a gesture recognition accuracy of $0.85$, thereby highlighting the crucial impact of \emph{gesture recognition errors} on learning performance, which ``confuses'' the agent by updating the wrong bandit's $Q$- and $n$ value. 

\begin{figure}[t]
	\centering
	\includegraphics[width=\columnwidth]{figures/sim04_recsucc085.png}
	\includegraphics[width=\columnwidth]{figures/sim04_recsucc085_2.png}
	\includegraphics[width=\columnwidth]{figures/sim04_recsucc085_3.png}
	\label{fig:sim04}
	\caption{Simulation result for a \texttt{UserAgent} generated with parameters $\mathcal{P}_{success} = 0.8$, $\mathcal{P}_{expressivity} = 0.9.$, gesture recognition error rate = $0.15$. Visualization settings are the same as in Fig.~\ref{fig:sim01}. Time steps with \textbf{\emph{gesture recognition errors}} are highlighted with \textbf{grey background}. As we can observe, \emph{gesture recognition errors} lead to updating the wrong bandit's $Q$ and $n$ value.}
\end{figure}

We can finally quantify the impacts of these \emph{cognitive mismatch} errors on the overall learning performance: We perform 100 simulated experiments using the following parameters: Condition $C_1$ = [$\mathcal{P}_{success} = 0.8$, $\mathcal{P}_{expressivity} = 0.9.$, gesture recognition accuracy = $1$], $C_2$ = [$\mathcal{P}_{success} = 0.8$, $\mathcal{P}_{expressivity} = 0.4.$, gesture recognition accuracy = $1$], $C_3$ =  [$\mathcal{P}_{success} = 0.6$, $\mathcal{P}_{expressivity} = 0.9.$, gesture recognition accuracy = $1$], each experiment consisting of $n=30$ trials, yielding accuracies on perfectly learned mappings (i.e., 3 of 3 gesture-mappings are correct) of $0.65$,  $0.62$ and $0.2$, respectively. Apparently, whereas \emph{expressivity} does not have substantial effects, the proportion of \emph{erroneous feedback} significantly impacts learning, leading to a substantial drop in learning performance. Similarly, in our simulation setting assuming imperfect gesture recognition, by assuming a gesture recognition accuracy of $0.85$, involving 100 simulated experiments involving a \texttt{UserAgent} with parameters [$\mathcal{P}_{success} = 0.8$, $\mathcal{P}_{expressivity} = 0.9.$] each experiment consisting of $n=30$ trials, performance drops to $0.2$.

Note that this is a very strict evaluation, since we require \emph{all} gesture-action-mappings to be learned correctly - results would be better if we analyzed each gesture separately and averaged the results. Also, we do not account for the different number of trials spent on learning each gesture (our \texttt{UserAgent} just uses a random uniform gesture selection strategy, which might result in experimental runs where some gestures have receive a rather low number of actual trials) -- results will be better if the agent uses a more informed gesture selection strategy.

Despite the overly simplistic assumptions and data generation, these initial experiments suggest that the learned action values frequently converge to the true underlying action mapping after a few trials only. The more sources of errors we introduce (wrong feedback given/recognized, wrong gesture recognized), the longer the process takes to converge towards the correct action, or does actually converge towards an incorrect action.
We can regard these experiments as a \emph{baseline} for studying the impact of these error sources. In realistic settings, we would expect better results for this learning process and faster convergence, since
\begin{itemize}
\item the \textsc{fer} outputs obtained from the real drone camera stream show that deliberate emotional responses typically tend to be much more nuanced than the simplistic distributions generated in these experiments

\item in our experiments, the \texttt{UserAgent} \textbf{randomly} samples the gestures. However, for interactions with real users, we can expect that the user will select gestures \textbf{intentionally} (e.g., by focusing on those gestures for which the drone has not learned the correct mapping yet). In general, we can expect that the user will also adapt her/himself to the drone's responses (e.g., by adapting her/his emotional responses based on the drone's performance), i.e., we might expect to observe a \emph{mutual learning} process here (as the user also learns how the drone reacts to their feedback and correspondingly might adapt their behavior).

\end{itemize}
Ideally, by recording and analyzing these experiments, further interesting findings might be derived on what might be crucial factors for a successful human-drone teaming (e.g., our human participants do not know whether the drone has recognized the wrong gesture or wrongly interpreted their feedback, but will have to interpret the drone's actions somehow. However, we could retrospectively classify these error sources later on by investigating the drone's log, and correlate this with the users' reactions and performance.)

Issues to further investigate and optimize for this experimental setting:

Assumptions and computations need to be adapted to meet the real ranges and probability distributions obtained from the drone's video stream. 

One crucial limitation will be to tweak settings to **minimize the amount of required interaction time**. I.e., Users' attention and engagement will likely decrease if the 

- feedback time window and
- the number of trials required for the drone to learn the successful mapping

will be too large. Thus, it will be required to pinpoint in further "physical experiments" what constitutes "agreeable" settings for the human participant, and tweak the learning process towards this (it might be necessary to find the "sweet spot" between limiting the amount of interactions required with the user while still achieving a more or less stable learning convergence).  
